"Hello, is this Anna?": Unpacking the Lifecycle of Pig-Butchering Scams

Pig-butchering scams have emerged as a complex form of fraud that combines elements of romance, investment fraud, and advanced social engineering tactics to systematically exploit victims. In this paper, we present the first qualitative analysis of pig-butchering scams, informed by in-depth semi-structured interviews with $N=26$ victims. We capture nuanced, first-hand accounts from victims, providing insight into the lifecycle of pig-butchering scams and the complex emotional and financial manipulation involved. We systematically analyze each phase of the scam, revealing that perpetrators employ tactics such as staged trust-building, fraudulent financial platforms, fabricated investment returns, and repeated high-pressure tactics, all designed to exploit victims' trust and financial resources over extended periods. Our findings reveal an organized scam lifecycle characterized by emotional manipulation, staged financial exploitation, and persistent re-engagement efforts that amplify victim losses. We also find complex psychological and financial impacts on victims, including heightened vulnerability to secondary scams. Finally, we propose actionable intervention points for social media and financial platforms to curb the prevalence of these scams and highlight the need for non-stigmatizing terminology to encourage victims to report and seek assistance.

==> 04_Phases.tex <==
\section{Lifecycle of Pig-Butchering Scams}
\label{sec:phases}

Pig-butchering is a complex and multifaceted fraud that unfolds in a series of carefully orchestrated steps, each designed to progressively manipulate the victim on emotional, psychological, and financial levels. The scam begins with the scammer making initial contact and establishing an emotional bond, then luring the victim into fraudulent investments under the guise of a promising opportunity. The scammer gradually escalates the stakes by fostering the victim's trust and dependency, pressuring them to make larger investments, and ultimately disappearing with the funds. In some cases, scammers reappear in an attempt to extract additional value from their victims. In this section, we provide a detailed breakdown of each phase, illustrating how these scams operate and the sophisticated tactics scammers employ to deceive their victims.

\subsection{The Lure}
This is the initial step in the pig-butchering scam, during which the scammer establishes contact with the intended victim. This phase is characterized by the creation of a carefully crafted and seemingly authentic persona. Victims are lured through social media platforms, dating applications, or unsolicited messages on popular messaging services. 

\noindent \textbf{Cold Texts.}
A significant proportion of participants ($n=18$, 69.2\%) reported that the initial contact with the scammer was through unsolicited messages via SMS, WhatsApp, or other messaging applications, where the scammer pretended to have entered an incorrect number. The first message of the form \textit{``Hello, is this} X\textit{"}, where \textit{X} was a random name. After being corrected by the victim, they would apologize but still introduce themselves and ask to continue the conversation. 

\noindent \textbf{Dating Apps.}
6 participants (23\%) were approached on dating platforms (2 via Tinder, 3 via Bumble, and 1 via Hinge). Scammers created attractive profiles, often featuring professionally taken photographs and bios highlighting shared interests with potential victims. Once a match was made, the scammers initiated conversations that quickly became personal, and attempted to move them off-platform on a messaging service like WhatsApp or Telegram.

\noindent \textbf{Social Media.}
A smaller segment ($n=2$) encountered scammers through social media platforms (1 each via Instagram and LinkedIn). Scammers would send connection requests or follow the victims, often engaging by commenting on public posts, and initiate conversation via personal messages. Scammer profiles were carefully crafted and not obviously fake; \textit{P4} recounts: 
\begin{center}
    \textit{``...his LinkedIn profile was well-written, mentioned his projects and work experience in fair detail, and also had testimonials. He also had connections in the thousands.}
\end{center}

\begin{mdframed}[style=insightstyle]
Pig-Butchering scams begin with the scammer establishing contact with the victim through various online platforms. Scammers create convincing personas and use unsolicited messages or interactions on dating apps and social media to engage the target. This phase is characterized by the  construction of trust through seemingly incidental or calculated interactions.
\end{mdframed}

\subsection{The Bond}
Following the initial contact, the scam progresses into the \textit{Bond} phase, wherein the scammer attempts to build a deep emotional connection with the victim. They engage the victim in daily conversations and make a concerted effort to be involved in their lives. The scammer may share what seem to be intimate and personal details about their own life, fostering a sense of mutual trust and emotional closeness. The underlying goal during this phase is to make the victim feel that they are part of a genuine, caring relationship. This phase often spans several months, where the scammer patiently builds a relationship with the victim.

\noindent \textbf{Nature of Relationships. }
Scammers cultivated either business or romantic relationships with victims. The majority of participants ($n=16$, 61.5\%) developed what they believed to be romantic relationships with the scammers. These relationships were characterized by frequent communication, expressions of affection, and discussions about future plans together. The remaining 10 participants (38.5\%) participants were enticed through the prospect of business partnerships or mentorships. Scammers presented themselves as successful entrepreneurs or seasoned professionals willing to share their knowledge.

\noindent \textbf{Rapport Building Techniques. }
Scammers invested significant time in building rapport, with participants noting daily communication over several weeks or months. They shared personal stories ($n=8$, 30.7\%), discussed family and career aspirations ($n=11$, 42.3\%) and showed empathy towards the victims' experiences ($n=5$, 19.2\%). Scammers frequently used mirroring as a manipulation technique; 9 participants (34.6\%) noted that the scammer agreed with them, or reacted positively to any view of theirs. In the words of \textit{P8}:
\begin{center}
    \textit{``He agreed with my viewpoints on almost everything, from politics to lifestyle choices. It was like a perfect fit; we were on the same wavelength."}
\end{center}
Scammers also gradually disclosed personal information to build trust, sometimes sharing fabricated hardships or vulnerabilities, such as a challenging past ($n=4$, 15.38\%) or experiences with debt ($n=9$, 34.6\%).

\noindent \textbf{Trust Building Techniques. }
Some scammers went even a step further in order to build more trust with victims. 17 participants (65.38\%) reported that the scammer sent frequent pictures of themselves, and their surroundings. 7 participants (26.9\%) reported having audio calls, and 3 participants (11.5\%) video calls with the scammers; they were able to verify that the pictures sent matched with the person they spoke to on the video call. According to \textit{P2}:
\begin{center}
    \textit{``When I spoke to her on a video call, it was the same person from the photos. She was even wearing the dress that matched a photo she had sent earlier in the day."}
\end{center}

\noindent \textbf{Social Media. }
Scammers used well-designed social media profiles to keep up the appearance of a genuine personality, and to back up some of the claims they made to victims. 20 participants (77\%) reported having connected with the scammer on at least one other social media platform: Facebook~($n=10$, 38.46\%), Instagram~($n=14$,53.84\%), or X~($n=9$, 34.61\%). Participants reported that the profiles were consistent with the details that the scammer shared, and that this was an important factor in them believing that the scammer was in fact a genuine person. For example, \textit{P18} shared:
\begin{center}
    \textit{``She said she liked dogs, and there was a picture of her with her dog on her Instagram. She said she went to [university] and her LinkedIn profile did say that too. It seemed legitimate, there was no reason to think that it could be fake -- if she could be a scammer, so could any of my actual friends."}
\end{center}
\noindent We requested participants to share links or screenshots of associated social media profiles. In all, we were able to collect $53$ profiles from various sites like Facebook, X, and LinkedIn. However, on following the links, or searching for the profiles based on the screenshot, we were unable to find even one. Our suspicion is that scammers churned profiles, and dumped an identity/social media profile after a successful attack. Additionally, because considerable time has passed since the original scam, the profiles may also have been taken down by platforms. 

\noindent \textbf{Duration. }
The bond phase showed that scammers had tremendous patience; this phase lasted anywhere from 3 to 11 months before the scammer moved on to the next stage of the scam. Scammers spent a significant amount of time bonding with the victim, to cultivate a sense of trust. According to 20 participants (76.9\%), this led them to letting their guard down and dispel any suspicions about this being a scam; \textit{P5} commented: 
\begin{center}
    \textit{``She did not push me to invest, or ask for money. She seemed genuinely interested in me and we spoke for nearly 6 months before she even brought up investments; it all seemed so real and organic."}
\end{center}

\begin{mdframed}[style=insightstyle]
Scammers deepen the relationship by fostering emotional trust with the victim through regular, personal interactions. They often simulate a romantic or business relationship that feels genuine to the victim. Over time, the victim becomes emotionally dependent, making them more susceptible to manipulation. The scammers' goal is to establish a strong emotional connection that will facilitate later exploitation.
\end{mdframed}
\subsection{The Bait}
Once trust has been firmly established, the scammer proceeds to the \textit{Bait} phase, where they introduce the fraudulent opportunity that forms the crux of the pig-butchering scam.

\noindent \textbf{Introducing Investments. }
Scammers typically introduce cryptocurrency investment into the conversation in a casual manner, referring to it as an extra source of income ($n=15$, 57.7\%) or even a hobby ($n=3$, 11.5\%). They may claim to have insider knowledge or expertise in crypto trading ($n=19$, 73\%), or an investment consultant who manages their portfolio ($n=7$, 27\%). The bait is framed as an exclusive opportunity, often portrayed as an investment that is only available to a select few. 6 participants reported that the scammer described their investments in a manner aligned with the victims' circumstances, such as debts or future aspirations. In the words of \textit{P23}:
\begin{center}
    \textit{``When we were talking, I had mentioned that I have some student loan debt. She said that she also was in a lot of debt, but these investments have helped her pay off the debt, and start building her own wealth."}
\end{center}

\noindent \textbf{Providing Social Proof. }
Scammers provided fake screenshots or access to counterfeit investment platforms displaying impressive returns. 22 participants (84.6\%) were shown evidence of significant profits through fabricated screenshots. Scammers may also provide proof via testimonials; 5 participants (19.2\%) reported that the scammer showed them emails or message screenshots confirming successful returns on investments. Further, 4 participants (15.4\%) were also given emails and phone numbers of other supposed investors, so that they could act as references. Participant \textit{P20} says:
\begin{center}
    \textit{``He had a well-crafted LinkedIn profile, and several testimonials from other profiles that sung praises of his investment and market analytics skills. The other profiles looked real too; this was enough for me to trust him."}
\end{center}

\noindent \textbf{Leveraging FOMO. }
The scammer emphasizes the exclusivity and limited nature of the opportunity, thereby exploiting the victim's fear of missing out (FOMO). This approach is designed to make the victim feel privileged to be ``invited" into the scheme, which heightens the perceived legitimacy and desirability of the investment; 18 participants (69.2\%) reported that the scammer presented the investment guidance as secret or highly specialized. At this point, the victim, already emotionally invested and trusting of the scammer, is primed to believe that this opportunity is both genuine and lucrative.
\begin{mdframed}[style=insightstyle]
After a bond has been established, the scammer introduces a fraudulent investment opportunity, typically framed as a low-risk, high-reward endeavor, such as cryptocurrency trading. The scammer uses fabricated success stories and social proof to persuade the victim of the legitimacy of the offer. This phase is designed to exploit the trust and rapport built in earlier stages, positioning the scammer as a trusted financial advisor or insider.
\end{mdframed}

\subsection{The Feed}
During the \textit{Feed} phase, the scammer transitions from enticing the victim to actively extracting financial contributions.

\noindent \textbf{Fraudulent Investment Platforms. }
Scammers provide access to sophisticated-looking but fraudulent investment platforms or applications, and asked victims to sign up for an account. All the participants reported creating accounts on such websites. 11 participants (42.3\%) reported that the scammer helped them set up their accounts through step-by-step instructions; 5 (19.2\%) reported that there were even help articles or some form of customer support. These platforms were authentic-looking, and displayed real-time information, with  efforts taken to ensure that they resembled real websites. \textit{P22} says:
\begin{center}
    \textit{"[the site] was similar to what you would expect on an investment portfolio website; in fact, the prices of stocks and bitcoin also matched..."}
\end{center}
\noindent Similar to social media profiles, we attempted to analyze the fraudulent investment platforms. We were able to collect a list of $23$ apps/platforms from participants, but found that the websites were no longer active. Our hypothesis is that since it is trivial to purchase new domain names, scammers frequently change domains as an evasion tactic. 

\noindent \textbf{Initial Investments. }
The scammer typically begins by encouraging the victim to make a modest initial investment. Participants reported initial investments of \$20 -- \$125. This allowed the victim to test the waters without feeling at great risk, and it also provides an opportunity for the scammer to build credibility. To maintain the illusion of legitimacy, the scammer may manipulate fake trading platforms or falsify investment returns, making it appear as if the initial investment has yielded positive gains; all the participants saw significant gains in their initial investment (2x -- 5x). 3 participants (11.5\%) also reported being allowed to withdraw some amount, further convincing them of the credibility of the investments. As \textit{P1} says:
\begin{center}
    \textit{"I was skeptical, and put in only \$25, but it soon became \$100, just as she had predicted! I was able to withdraw it in the form of a gift card too -- the investment strategy seemed legitimate."}
\end{center}

\noindent \textbf{Escalating Investments. }
Scammers applied subtle pressure to reinvest profits rather than withdraw them. 23 participants (88.4\%) were encouraged to roll over their gains into new investments, so as to earn even more. As victims grew more comfortable, scammers suggested larger investments to achieve greater profits. According to 13 participants (50\%), victims were encouraged to use their 'profits' as leverage for higher-tier investment opportunities. All participants reported increasing their investment amounts significantly (\$3,500 -- \$65,00) by putting in more money. Participants also saw tremendous gains on their investments on the platform (2x -- 12x).

\noindent \textbf{Manipulation Techniques. }
Scammers maintained regular communication, celebrating the victim's 'successes' and reinforcing the notion of smart investing; 12 participants (46.1\%) received congratulatory messages whenever their account showed any gains. Scammers often claimed to be investing alongside the victims, fostering a sense of shared endeavor; they manipulated the investment platform so as to create this illusion, even 'lending' money if needed ($n=14$, 53.8\%). \textit{P14} recounts: 
\begin{center}
    \textit{"..there was this particular opportunity that had a \$1000 minimum, but I did not feel confident enough and had only \$500 in the account; she said she can front me the remaining amount (as it would be for our future together) -- and the amount really did arrive as a transfer to my account [on the platform]!"}
\end{center}
Further, according to 8 participants (30.7\%), scammers introduced complex investment strategies, using technical jargon to appear knowledgeable. Finally, all participants reported that scammers discouraged them from discussing investments with others, citing reasons like market confidentiality.
\begin{mdframed}[style=insightstyle]
    Scammers persuade victims to invest in fraudulent platforms that mimic legitimate financial services. Initial investments are typically small, with fabricated returns used to encourage further contributions. The scammer maintains ongoing communication, reinforcing the illusion of success and increasing the victim’s financial commitment by encouraging reinvestment of perceived gains.
\end{mdframed}


\subsection{The Squeeze}
In the \textit{Squeeze} phase, the scammer escalates the pressure on the victim to act with urgency. By this stage, the scammer has already secured the victim's trust and convinced them of the legitimacy of the investment scheme, making the victim highly susceptible to psychological manipulation. 

\noindent \textbf{Exclusive Deals. }
After continuing investments, all participants were presented with time-sensitive, high-return investment opportunities. Scammers claimed access to insider deals ($n=12$, 46.2\%) or initial coin offerings (ICOs) ($n=9$, 34.6\%) about to explode in value. These investments had minimum amounts, which were often large (in the tens of thousands). 18 participants(69.2\%) reported that they felt inclined to invest, because of the perceived returns so far.

\noindent \textbf{Pressure Tactics. }
To ensure the high investment, scammers increased the frequency and urgency of their messages. All participants reported receiving multiple messages or calls daily, emphasizing the need for immediate action. Scammers employed emotional manipulation, expressing disappointment or suggesting that the victim was missing out due to hesitation. 11 participants (42.3\%, for whom the relationship was of a romantic nature) also reported frustruation on the scammer's part; as \textit{P10} put it: 
\begin{center}
    \textit{``[she] got extremely angry, and asked me whether I was actually serious about settling down with her, and if so, why I wasn't making an effort to put in this money."}
\end{center}

\noindent \textbf{Continuing Investments. }
Scammers encouraged victims to ``re-invest" their gains, and add more funds rather than attempt to withdraw them. Exclusive opportunities as described above keep on occurring till the victim invests. The squeeze serves to drain any remaining financial resources the victim may have access to, pushing them to borrow money or liquidate other assets if necessary. 9 participants (34.6\%) reported that the scammer recommended using credit cards or applying for new credit cards so as to use credit to invest. 
The squeeze phase lasts for as long as the victim is willing to invest; participants reported continuing large investments and perceived profit for 1-7 months. By the end of this phase, the scammer aims to have extracted as much financial value as possible.

\begin{mdframed}[style=insightstyle]
    Once the victim is fully engaged, scammers escalate pressure by introducing time-sensitive, high-return investment opportunities, often requiring large additional investments. Emotional manipulation intensifies, with scammers leveraging the victim's trust and fear of missing out (FOMO) to secure further financial commitments. This phase aims to extract as much financial value as possible from the victim.
\end{mdframed}

\subsection{The Cut}
This phase marks the culmination of the pig-butchering scam, during which the scammer absconds with all of the victim's invested funds. The scammer transitions into the cut phase after they are convinced that they have squeezed the victims of the maximum amount possible. 

\noindent \textbf{Stalling Tactics. }
The cut phase typically begins when victims refuse to invest any more money, and attempt to withdraw funds. Scammers used several tactics to delay the withdrawal; 21 participants (80.8\%) discovered that they could suddenly no longer access their investment accounts. 10 participants (38.4\%) reported that the platforms displayed error messages or indicated that the account was under review. Some scammers went a step further; 16 participants reported that the platform asked for more money under the guise of withdrawal fees or taxes. 4 participants (15.4\%) fell for this and ended up paying. \textit{P19} says:
\begin{center}
    \textit{``At the time, I had [perceived] \$250k in the account, and when I attempted to withdraw it, they said that 30\% had to be paid as taxes. When I asked them to deduct it from the account, they refused, claiming that the money was tied up in crypto and government regulations needed taxes to be paid directly. I even chatted with a support representative on the site." }
\end{center}

\noindent \textbf{Complete Disappearance. }
After either paying fees for withdrawal, or refusing to do so, all but one participants reported the scammer ceasing all communication. Scammers blocked the victims on chat application (WhatsApp / Telegram), as well as any social media platforms they were connected on. Scammer accounts were likely deleted or deactivated; 18 participants (69.2\%) searched for the profiles using other accounts, but could not find them. \textit{P22} says:
\begin{center}
    \textit{``I used my sister's Instagram to look for her, but I couldn't find her profile. I also tried messaging her on WhatsApp using my sister's number, but the app said that this number wasn't on WhatsApp."}
\end{center}
\begin{mdframed}[style=insightstyle]
    After squeezing the victim as much as possible, scammers abscond with the victim’s funds, typically after the victim attempts to withdraw their investments. Scammers employ stalling tactics, such as claiming technical issues or additional fees, to delay withdrawal. Once the victim realizes they have been defrauded, the scammer cuts all communication, disappearing from both the financial platform and social media.
\end{mdframed}

\subsection{The Encore}
Even after disappearing, scammers may attempt an \textit{Encore} by re-engaging the victim for additional scams. This phase leverages the victim's desperation to recover their lost funds and exploits the emotional turmoil resulting from the initial scam. After extracting the money, encore scammers block the victim and disappear.

\noindent \textbf{Impersonation Scams. }
Scammers frequently impersonate law enforcement officials to re-establish contact with victims. They pose as detectives, federal agents, or members of cybercrime units investigating the original scam. 15 participants (57.7\%) reported receiving official-looking communications, complete with badges, case numbers, and legal jargon. 8 (30.7\%) reported that the supposed agent requested personal information under the guise of needing it for the investigation. According to \textit{P12}:
\begin{center}
    \textit{``I received an email from someone claiming to be an FBI agent, stating that they had found my account details when they took down the platform, and that they were closing in on the scammers who took my money. They asked for my bank statements and ID to 'verify' my case, and I complied without thinking twice."}
\end{center}
Further, 9 participants (34.6\%) reported that these fraudulent officials informed them that their funds have been located but require payment of legal fees or taxes to release them. Overall, 15 participants were victims of impersonation scams, and ended up paying additional amounts of \$120 -- \$1700. 

\noindent \textbf{Recovery Scams. }
Scammers, sometimes the original perpetrators or new opportunists, contact victims offering services to retrieve lost funds. 11 participants reported being contacted by such recovery experts. They present themselves as recovery specialists ($n=7$, 26.9\%) private investigators ($n=2$, 7.6\%), or legal professionals with expertise in financial fraud cases ($n=5$, 19.2\%). They typically request upfront fees for their services, citing costs for legal processes, court fees, or administrative expenses. Overall, 11 participants were approached with recovery scam offers. These scams can be highly sophisticated; \textit{P20} says:
\begin{center}
    \textit{``They had a website and a case management portal; there were many different professionals within the company; a case manager, a lawyer, a digital forensics expert...."}
\end{center}

\noindent \textbf{Legal Threats. }
Scammers may also employ legal threats to intimidate victims into making additional payments. They impersonate lawyers ($n=4$, 15.4\%), debt collectors ($n=1$, 3.8\%), or officials from regulatory agencies ($n=2$, 8.6\%), claiming that the victim has breached contracts or violated laws through their previous investment activities. The threats typically include demands for immediate payment to avoid lawsuits, arrests, or damage to credit ratings. Scammers may threaten to report the victim to authorities for participating in illegal investment schemes or non-payment of taxes. \textit{P21} reported:
\begin{center}
    \textit{``I received an email from the platform saying that they were owed some fees from me, and if I do not comply, then they would be filing an official complaint with the IRS for tax evasion. "}
\end{center}
Overall, 7 participants reported being contacted with legal threats; however, fortunately, none of them fell for it. 
\begin{mdframed}[style=insightstyle]
    In some cases, scammers re-engage victims by posing as law enforcement or recovery agents, offering assistance in recovering lost funds for a fee. This phase exploits the victim’s emotional vulnerability and desperation, further compounding their financial losses. 
\end{mdframed}



